Modelling Interrelations Between Agile Practices: The Agile Map

Agile methods are defined through guidelines comprising various practices intended to enable agile ways of working. These guidelines further comprise a specific set of agile practices aiming to enable teams for an agile way of working. However, due to its wide-spread use in practice we know that agile practices are adopted and tailored intensively, which lead to a high variety of agile practices in terms of their level of detail. Problem: A high variety of agile practices can be challenging as we do not know how different agile practices are interrelated with each other. To be more precise, tailoring and adopting agile practices may lead to the challenge, that the combinatorial use of several agile practices can only be successful to a limited extent, as practices support or even require each other for a effective use in practice. Objective: Our study aims to provide an enabler for this problem. We want to identify interrelations between agile practices and describe them in a systematic manner. Contribution: The core contribution of this paper is the Agile Map, a theoretical model describing relations between agile practices following a systematic approach aiming to provide an overview of coherences between agile practices. The model aims to support practitioners in selecting and combining agile practices in a meaningful way.

==> thomas.tex <==
\section{no sure}

In the conference paper "The Integrated List of Agile Practices - A Tertiary Study", the 38 essential agile practices were synthesized from 944 agile practices. These formed the basis for the study of the intermediate relationships between the agile practices. The aim is to enable companies to detach themselves from specific agile methods and create their own agile framework consisting of the agile practices that best suit the company.

In the course of this, the agile practices were first described in terms of content. Their intermediate relationships then emerged from the content descriptions. This revealed that these relationships can be classified into four relationship types.

The specialization relation describes a subset relationship. The source element therefore represents a special form of the target element.

The support relation states that the source element has a supporting effect on the target element. It is used when the target element offers greater added value if the source element is also used. The relationship can be both unidirectional and bidirectional.

The requirement relation states that the target element must also be used for the effective implementation of the source element. The mandatory character is also given in this context if the source element can be used without the target element, but this contradicts the basic idea of an agile way of working. The relationship is always unidirectional.

The alternative relation states that the source and target elements are practices that are similar in their basic features and can therefore be used as alternatives to each other.

The result was an agile map that shows these coherences.

In addition to the coherences, the content-related investigations have shown that agile practices are often not clearly described or defined. It can be assumed that this is one of the reasons for the large number of agile practices that exist today in the context of modern software development methods.

In order to develop a more generally valid model of agile practices and their coherence, it is first necessary to precisely specify and classify the existing practices.

In the second step, the coherence of each agile practice with other agile practices must be broken down, as shown in the agile map. In the course of this, the requirement relation is particularly important, as it shows which agile practices must inevitably be used together.

In the third step, the principles and values described by the »Agile Alliance« in its »Manifesto for Agile Software Development«  are used to specify the core objectives of agile software development. (The core objectives that we have seen so far are service provision (sp), process optimization (po) and the exchange of knowledge and experience (ke)).

The fourth step involves researching which agile practices are suitable for implementing which of the goals defined in step three.
With the help of this systematization, it should be possible for companies to select specific agile practices, which can then be put together very individually into an iterative-incremental process. To this end, it may be helpful to create generally applicable rules for creating such a process from specific agile practices.

This should also make it possible to replace individual agile practices (or a group) of agile practices if the company determines that they do not optimally support the process.


